Optimal Bit and Power Loading for OFDM Systems with Average BER and Total Power Constraints

In this paper, a novel joint bit and power loading algorithm is proposed for orthogonal frequency division multiplexing (OFDM) systems operating in fading environments. The algorithm jointly maximizes the throughput and minimizes the transmitted power, while guaranteeing a target average bit error rate (BER) and meeting a constraint on the total transmit power. Simulation results are described that illustrate the performance of the proposed scheme and demonstrate its superiority when compared to the algorithm in [1].

==> TEMP.tex <==
\begin{eqnarray}
\textup{subject to} \quad g(\mathbf{p},\mathbf{b}) = \: 0.2 \: \sum_{i=1}^{N}b_i \: \textup{exp}\left ( \frac{- 1.6 \: \mathcal{C}_i \mathcal{P}_i}{2^{b_i} - 1} \right ) \nonumber\\  - \: \textup{BER}_{th} \: \sum_{i=1}^{N}b_i \leq 0, \quad i = 1, ..., N, \nonumber \\ \label{eq:ineq_const}
\end{eqnarray}



\mathcal{L}(\mathbf{p},\mathbf{b},\mathcal{Y}, \lambda) &{} = {}& \mathcal{F}(\mathbf{p},\mathbf{b}) + \lambda \: \mathcal{G}(\mathbf{p},\mathbf{b},\mathcal{Y}), \nonumber \\
 &{} = {}& \alpha \sum_{i = 1}^{N}\mathcal{P}_i - (1-\alpha)\sum_{i = 1}^{N}b_i \nonumber \\ 
& & + \lambda \: \Bigg[ 0.2 \: \sum_{i=1}^{N}b_i \: \textup{exp}\left ( \frac{- 1.6 \: \mathcal{C}_i \mathcal{P}_i}{2^{b_i} - 1} \right ) \nonumber \\ 
& & \hspace{2cm} - \: \textup{BER}_{th} \: \sum_{i=1}^{N}b_i + \mathcal{Y}^2 \Bigg], 
%0.2 \: \textup{exp}\left ( \frac{- 1.6 \: \mathcal{C}_i \mathcal{P}_i}{2^{b_i} - 1} \right ) - \textup{BER}_{th,i} \nonumber \\ 
%& & \hspace{4.5cm}+ \mathcal{Y}_i^2\Bigg],


\setlength{\arraycolsep}{0.0em}
\begin{eqnarray}
\frac{\partial \mathcal{L}}{\partial \mathcal{P}_i} &{} = {}& \alpha - 0.2 \times 1.6 \: \lambda \frac{b_i \: \mathcal{C}_i}{2^{b_i}-1} \: \textup{exp}\left ( \frac{- 1.6 \: \mathcal{C}_i \mathcal{P}_i}{2^{b_i} - 1} \right ) = 0, \label{eq:eq1}\\
\frac{\partial \mathcal{L}}{\partial b_i} &{} = {}& -(1 - \alpha) + \lambda \Bigg[0.2 \: \textup{exp}\left ( \frac{- 1.6 \: \mathcal{C}_i \mathcal{P}_i}{2^{b_i} - 1} \right ) \nonumber \\ & & \times \bigg[1+ 1.6 \times \ln(2) \frac{\mathcal{C}_i \mathcal{P}_i b_i 2^{b_i}}{(2^{b_i}-1)^2}\bigg] - \textup{BER}_{th} \Bigg] = 0, \label{eq:eq2}\\
\frac{\partial \mathcal{L}}{\partial \lambda} & = & 0.2 \: \sum_{i=1}^{N}b_i \: \textup{exp}\left ( \frac{- 1.6 \: \mathcal{C}_i \mathcal{P}_i}{2^{b_i} - 1} \right ) - \: \textup{BER}_{th} \: \sum_{i=1}^{N}b_i \nonumber \\ & & \hspace{5.5cm} + \mathcal{Y}^2 = 0, \label{eq:eq3}\\
\frac{\partial \mathcal{L}}{\partial \mathcal{Y}} & = & 2\lambda \mathcal{Y} = 0. \label{eq:eq4}
\end{eqnarray}
